Cooperative Vehicle Speed Fault Diagnostics and Correction

Reliable estimation (or measurement) of vehicle states has always been an active topic of research in the automotive industry and academia. Among the vehicle states, vehicle speed has a priority due to its critical importance in traction and stability control. Moreover, the emergence of new generation of communication technologies has brought a new avenue to traditional studies on vehicle estimation and control. To this end, this paper introduces a set of distributed function calculation algorithms for vehicle networks, robust to communication failures. The introduced algorithms enable each vehicle to gather information from other vehicles in the network in a distributed manner. A procedure to use such a bank of information for a single vehicle to diagnose and correct a possible fault in its own speed estimation/measurement is discussed. The functionality and performance of the proposed algorithms are verified via illustrative examples and simulation results.

==> Section5.tex <==
First, each vehicle $v_i$ applies a distributed algorithm to gather the information (velocities) of all of the vehicles in the network via using only local information exchange (with the vehicles in its communication range, called neighbors). These information contains positions,  longitudinal velocities and accelerations of other vehicles in the network. Two different versions of this algorithm are proposed in this paper. In the first algorithm, it is assumed that there is no failure in vehicle communications and in the second algorithm, we assume that some of the vehicles fail to communicate and disseminate their information properly. 

    
    \item[(2)] \textbf{Speed Fault Diagnosis:}
    
    After finding the values for other vehicles, vehicle $v_i$ does the following error computation:
    \begin{multline}
    e_i^j=\kappa_1\left(u_{ij}-\int (a_{ij}) dt \right) 
    +\kappa_2\left(u_{ij}-\frac{d(p_{ij})}{dt}  \right)
    \label{eqn:partial}
\end{multline}
where $\kappa_1, \kappa_2>0$ are some design constants and $p_{ij}$, $u_{ij}$ and $a_{ij}$ are relative distance, velocity and acceleration of vehicles $v_i$ and $v_j$.  In order for $v_i$ to be able to analyze the error information  \eqref{eqn:partial}, it is required to have access to enough information from many other vehicles, which are obtained from step (1). 

    \item[(3)] After calculating error parameter $e_i^j$ by vehicle $v_i$ for all vehicles $v_j$ in the network, it makes a logical comparison. If $e_i^j$ is nonzero for only a specific vehicle $v_j \in \mathcal{V}$, then the velocity $u_j$ is faulty. If $e_i^j$ is nonzero for (almost) all vehicles $v_j \in \mathcal{V}$, then the velocity $u_i$ is faulty.  
